With Great Speed Come Small Buffers: Space-Bandwidth Tradeoffs for Routing

We consider the Adversarial Queuing Theory (AQT) model, where packet arrivals are subject to a maximum average rate $0\le\rho\le1$ and burstiness $\sigma\ge0$. In this model, we analyze the size of buffers required to avoid overflows in the basic case of a path. Our main results characterize the space required by the average rate and the number of distinct destinations: we show that $O(k d^{1/k})$ space suffice, where $d$ is the number of distinct destinations and $k=\lfloor 1/\rho \rfloor$; and we show that $\Omega(\frac 1 k d^{1/k})$ space is necessary. For directed trees, we describe an algorithm whose buffer space requirement is at most $1 + d' + \sigma$ where $d'$ is the maximum number of destinations on any root-leaf path.

==> basic-alg-tree.tex <==
In this section we consider the case where $G$ is a directed tree. That 
is, the underlying topology of $G = (V, E)$ is a tree. There is a 
pre-specified root $r \in V$, and all edges are directed toward the 
root. We describe a simple algorithm that requires buffers of size $1 + 
d' + \sigma$ for all rates $\rho \leq 1$ and \emph{destination depth} 
$d'$ (defined below). By Thm.~\ref{thmLB}, this space requirement is 
optimal for rates $\rho$ satisfying $1/2 < \rho \leq 1$. We break the 
description into two parts.  We first consider the case where all 
packets have a common destination: The algorithm ``Peak-to-Sink'' 
(\PTS) solves it using the best possible buffer space of $2 + \sigma$ 
packets. This preliminary result matches the main algorithmic result 
of~\cite{Miller2016} with a significantly simplified algorithm and 
analysis. We then generalize the algorithm to the case of arbitrary 
destinations.

The orientation of edges $e \in E$ toward $r$ induces a partial order 
denoted $\prec$.
%, called the \dft{tree order} on $V$. 
Specifically, for $u, v 
\in V$, we have $u \prec v$ if and only if $v$ is on the unique path 
from $u$ to $r$. Thus, leaves are minimal with respect to $\prec$, 
%(in the sense that if $v$ is a leaf, there is no $u$ satisfying $u 
%\prec v$), 
and the root $r$ is maximal. By extension, given a configuration $L$ of 
$G$, $\prec$ induces a partial order on packets, where $P \prec P'$ if 
$P \in L(u)$, $P' \in L(v)$ with $u \prec v$.



\subsection{Single destination}

Suppose first that all packets have destination $r$, the root of $G$.  
We say that a packet $P \in L^t(v)$ is \dft{bad} if it is
stored at position $p \geq 2$, and $L^t(v)$ is bad if $\abs{L^t(v)} 
\geq 2$ (i.e., if it contains a bad packet). The $\PTS$ algorithm 
selects a maximal set of ``farthest'' bad buffers from the root, and 
activates the union of paths from these buffers to the root. The 
following definition formalizes this idea.

\begin{dfn}
  \label{dfn:min-antichain}
  Let $\calB^t \subseteq V$ be the set of bad buffers at time $t$. We call $\calP \subseteq \calB^t$ a \dft{min-antichain} if the following hold:
  \begin{compactenum}
  \item $\calP$ is an antichain with respect to $\prec$; that is, for all $u, v \in \calP$, $u \nprec v$ and $v \nprec u$.
  \item For every $v \in \calB$ either $v \in \calP$ or there exists $u \in \calP$ such that $u \prec v$.
  \end{compactenum}
\end{dfn}

Given $\calB^t$, there is a unique min-antichain, $\min(\calB^t)$, defined by
\(
\min(\calB^t) = \set{u \in \calB^t \sucht \forall v \in \calB^t, v \nprec u}.
\)
Our generalization of $\PTS$ activates buffers as follows: Let $\calP = \min(\calB^t)$. Then define $\calA$ to be
\(
\calA = \bigcup_{u \in \calP} \Path(u, r),
\)
where $\Path(u, v)$ returns the set of vertices on the unique path from $u$ to $v$ in $G$. More concisely, $\PTS$ activates every buffer $v \in V$ such that there exists a bad buffer $u$ with $u \preceq v$. We state the performance of this variant of $\PTS$ in the following.

\begin{prop}
  \label{prop:tree-pts}
  Suppose $G$ is a directed tree, $A$ is a $(\rho, \sigma)$-bounded adversary with $\rho \leq 1$, and all packets $P \in A$ have destination $r$. Then then maximum buffers size is at most $2 + \sigma$.
\end{prop}

To prove Proposition~\ref{prop:tree-pts}, we bound the number of bad packets ``behind'' any node $v \in V$ by $\xi^t(v) + 1$ during any step of the algorithm.

\begin{dfn}
  Let $v \in V$. Let $G_v = (U_v, E_v)$ denote the (directed) subtree of $G$ rooted at $v$, so that $U_v = \set{u \in V \sucht u \preceq v}$. For each $v \in V$ we define $\beta^t(v) = \max\set{\abs{L^t(v)}-1, 0}$ to be the number of bad packets in $v$. The \dft{badness} of $v$ is
  \(
  B^t(v) = \sum_{u \in U_v} \beta^t(u).
  \)
  That is, $B^t(v)$ is the number of bad packets whose paths contain $v$.
\end{dfn}

\begin{lem}
  \label{lem:tree-bad-decrease}
  Let $L^t$ be a configuration and $\calA$ the set of activated nodes described above. For any $v \in V$, let $B^{t+}(v)$ denote the badness of $v$ immediately after forwarding. Then
  \(
  B^{t+}(v) \leq \max\set{B^t(v) - 1, 0}.
  \)
\end{lem}
\begin{proof}%[Proof of Lemma~\ref{lem:tree-bad-decrease}]
  We argue by induction on the depth $D_v$ of $G_v$. For $D_v = 0$, $v$ is a leaf so that $v$ does not receive any packets. Therefore, $B^{t+}(v) \leq \max{B^t(v) - 1, 0}$. Now suppose the holds for all depths $D' < D_v$. If $B^{t}(v) = 0$, then $v$ neither sends, nor receives any packets as no node $u \in U_v$ is activated. Consider the case where $B^t(v) \geq 1$. Let $u_1, u_2, \ldots, u_k$ denote the children of $v$ satisfying $B^t(u_i) \geq 1$ for $i = 1,2,\ldots, k$. By the inductive hypothesis, the badness of each $u_i$ decreases by at least $1$ as a result of forwarding. Therefore we compute
  \begin{align*}
    B^{t+}(v) &= \sum_{i = 1}^k B^{t+}(u_i) + \paren{\beta^{t+}(v) - \beta^t(v)} + \beta^t(v) \leq \beta(v) + \sum_{i = 1}^{k} (B^{t}(u_i) - 1) + \paren{\beta^{t+}(v) - \beta^t(v)}\\ &=\beta(v) + \sum_{i = 1}^{k} B^{t}(u_i) + \paren{\beta^{t+}(v) - \beta^t(v)} - k = B^t(v) + \paren{\beta^{t+}(v) - \beta^t(v)} - k \leq B^t(v) - 1.
  \end{align*}
  The final inequality $\beta^{t+}(v) - \beta^t(v) - k \leq -1$ holds because $v$ receives at most $k$ packets: either $\abs{L^t(v)} = 0$ and at most $k - 1$ of the received packets become bad, or $\abs{L^t(v)} \geq 1$ in which case $v$'s load (hence $\beta(v)$) increases by at most $k - 1$.
\end{proof}

\begin{proof}[Proof of Prop.~\ref{prop:tree-pts}]
  We argue by induction on $t$ that for all $v$ $B^t(v) \leq \xi^t(v) + 1$ and $B^{t+}(v) \leq \xi^t(v)$. The proposition then follows from Part~(1) of Lemma~\ref{lem:excess}, as $\xi^t(v) \leq \sigma$ for all $t$. To prove the inductive step of the claim, suppose $B^{(t-1)+}(v) \leq \xi^t(v)$. Then by Part~(2) of Lemma~\ref{lem:excess}, $N_{\{t\}}(v) \leq \xi^t(v) - \xi^{t-1} + \rho$. Since the badness of $v$ increases by at most $N_{\{t\}}(v)$, the inductive hypothesis gives $B^t(v) \leq \xi^t(v) + \rho \leq \xi^t(v) + 1$. By Lemma~\ref{lem:tree-bad-decrease}, we have $B^{t+}(v) \leq \max\set{B^t(v) - 1, 0} \leq \xi^t(v)$. Since each $v$ contains at most one non-bad packet, we have $L^t(v) \leq 1 + B^t(v) \leq 2 + \sigma$, as desired.
\end{proof}





\subsection{Multiple destinations}

We describe a generalization $\PTS$ to trees with multiple possible destinations. We call the generalize algorithm \dft{Parallel Peak-to-Sink} ($\PPTS$). Let $W = \set{w_1, w_2, \ldots, w_d}$ be a set of possible destinations of packets. We assume that the sequence $w_1, w_2, \ldots, w_d$ is a topological sorting of $W$ so that $w_i \prec w_j$ implies that $i < j$. We partition $L^t(v)$ into pseudo-buffers $\set{L_k^t(v) \sucht k \in \Seq{d}}$, where $L_k^t(v)$ stores packets destined for $w_k$. Badness of pseudo-buffers is defined as follows:
\[
\beta_k^t(v) = \max\set{\abs{L_k^t(v)} - 1, 0}, \qquad B_k^t(v) = 
\sum_{u \in U_v} \beta_k^t(u), \qquad B^t(v) = \sum_{k \in \Seq{d}} 
B_k^t(v).
\]
We call $B_k^t(v)$ the \dft{$k$-badness} of $v$ at time $t$. We denote $\calB_k^t = \set{v \in V \sucht \beta^t_k(v) \geq 1}$ to be the set of nodes containing $k$-bad pseudo-buffers.

The $\PPTS$ algorithm for directed trees activates $k$-pseudo-buffers in descending order (of $k$) as described in Algorithm~\ref{alg:tree-pp2s}. More specifically, for $k = d, d-1, \ldots, 1$, $\PPTS$ looks for bad packets with destination $w_k$. For each bad buffer $u$, $\PPTS$ activates all $k$-pseudo-buffers along $\Path(u, w_k)$ that have not previously been activated (this round) for some $k' \geq k$. A straightforward generalization of the proof of Lemma~\ref{lem:tree-bad-decrease} yields the following (proven in the appendix).

\begin{lem}
  \label{lem:ppts-bad-decrease}
  Let $v \in V$ be buffer with $B^t(v) \geq 1$. Then there exists $k' \in [d]$ such that $L_{k}^t(v) \in \calA$. For all $k \in [d]$ we have
  \[
  B^{t+}_k(v) \leq
  \begin{cases}
    B^{t}_k(v) &\text{if } k \neq k'\\
    B^{t}_k(v) - 1 &\text{if } k = k' 
  \end{cases}
  \]
  Therefore, $B^{t+}(v) \leq B^t(v) - 1$.
\end{lem}

In order to quantify the performance of Algorithm~\ref{alg:tree-pp2s}, we define the \dft{destination depth} $d' = d'(G, W)$ of $G$ with destinations $W$ to be the length of the longest chain of destinations in $W$. That is,
\[
d' = \max\set{s \sucht \exists  w_1, w_2, \ldots, w_s\in W, w_1 \prec w_2 \prec \cdots \prec w_s}.
\]
Note that $d' \leq \min\set{d, D}$ where $D$ is the depth of $G$.

\begin{thm}
  \label{thm:tree-ppts}
    Let $A$ be any $(\rho, \sigma)$-bounded adversary such that all packets have destinations in $W$. Then the maximum buffer usage of $\PPTS$ is at most $1 + d' + \sigma$.
\end{thm}

\begin{wrapfigure}{r}{.45\textwidth}
  \begin{minipage}{.45\textwidth}%\vspace{-8mm}
    \begin{algorithm}[H]\small
      \caption{$\PPTS(G, W)$ Step}
      \label{alg:tree-pp2s}
      \begin{algorithmic}[1]
        \STATE $\calA \leftarrow \varnothing$
        \FOR{$k\gets d-1$ \Downto $0$}
        \STATE $\calP \leftarrow \min(\calB^t_k)$
        \STATE $\calA_k \leftarrow \paren{\bigcup_{u \in \calP} \set{L_k(v) \sucht v \in \Path(u, w_k)}} \setminus \set{L_k(v) \sucht \exists L_{k'}(v) \in \calA}$
        \STATE $\calA \leftarrow \calA \cup \calA_k$ 
        \ENDFOR
        \STATE every active (nonempty) pseudo-buffer in $\calA$ 
        forwards a packet
      \end{algorithmic}
    \end{algorithm}
  \end{minipage}
\end{wrapfigure}

The proof of Thm.~\ref{thm:tree-ppts} is identical to the proof of Prop.~\ref{prop:tree-pts}, except that we employ Lemma~\ref{lem:ppts-bad-decrease} (instead of Lemma~\ref{lem:tree-bad-decrease}) to show that $B^t(v) \leq \xi^t(v) + 1$ for every $v$ and $t$. Thm.~\ref{thm:tree-ppts} follows by observing that each $v$ contains at most $d'$ non-bad packets, so its load is at most $d' + B^t(v) \leq d' + \sigma + 1$.

